Automatically Dismantling Online Dating Fraud

Online romance scams are a prevalent form of mass-marketing fraud in the West, and yet few studies have addressed the technical or data-driven responses to this problem. In this type of scam, fraudsters craft fake profiles and manually interact with their victims. Because of the characteristics of this type of fraud and of how dating sites operate, traditional detection methods (e.g., those used in spam filtering) are ineffective. In this paper, we present the results of a multi-pronged investigation into the archetype of online dating profiles used in this form of fraud, including their use of demographics, profile descriptions, and images, shedding light on both the strategies deployed by scammers to appeal to victims and the traits of victims themselves. Further, in response to the severe financial and psychological harm caused by dating fraud, we develop a system to detect romance scammers on online dating platforms. Our work presents the first system for automatically detecting this fraud. Our aim is to provide an early detection system to stop romance scammers as they create fraudulent profiles or before they engage with potential victims. Previous research has indicated that the victims of romance scams score highly on scales for idealized romantic beliefs. We combine a range of structured, unstructured, and deep-learned features that capture these beliefs. No prior work has fully analyzed whether these notions of romance introduce traits that could be leveraged to build a detection system. Our ensemble machine-learning approach is robust to the omission of profile details and performs at high accuracy (97\%). The system enables development of automated tools for dating site providers and individual users.

==> sections/core-old.tex <==

% -----------------------------------------------
\section{Classifying False Profiles}
% -----------------------------------------------
\label{sec:core}

We now introduce our approach to systematize the identification of false profiles
(\S\ref{sec:core:overview}). 
We next describe our proposed set of features (\S\ref{sec:core:fengineering}),
which is strongly motivated by the findings reported above. 
As not all profiles contain the same information, we then present three independent 
classifiers that are triggered accordingly; and we finally show how to ensemble 
and properly balance the different predictions to provide one single decision
(\S\ref{sec:core:model}). 



% ::::::::::::::::::::::::: % 
\subsection{Overview of Our System}
\label{sec:core:overview}
% ::::::::::::::::::::::::: % 

A high-level view of our system can be obtained from Figure \ref{fig:architecture-general}. 
The system is first trained using a dataset of real and scam profiles. The goal of 
this phase is to obtain the following key elements that will later be used to 
identify fraudsters:

\begin{comment}
\begin{figure*}[t]
\includegraphics[width=\textwidth, trim = 35 325 170 90, clip]{architecture-system}
\caption{Architecture of the proposed system.}\label{fig:architecture-system}
\end{figure*}
\end{comment}


\begin{enumerate}
\item[(i)] A set of prediction models $\mathcal{P} = \set{P_1, \ldots, P_i}$ that output the probability 
$$\theta_i(\phi_1, \ldots, \phi_n) = P_i[X=\texttt{scam}\mid(\phi_1, \ldots, \phi_n)]$$
of each profile $X$ being \texttt{scam} given a feature vector $(\phi_1, \ldots, \phi_n)$ obtained from different sections $i$ of the profile. 

\item[(ii)] A weighted model 
$$f(\mathcal{P}) = \sum w_i \cdot P_i $$
that combines all individual predictions in $\mathcal{P}$. Here, each individual 
classifier $P_i$ is weighted by $w_i$ according to the accuracy given on a validation 
set that is different from the training one. This will also serve as a way to 
calibrate individual probabilities. The final classifier will then output a decision 
based on a votation such that 
$$
f =
\begin{cases}
\texttt{scam} & \text{if~} f(\mathcal{P}) < \tau)\\
\texttt{real} & \text{otherwise,}
\end{cases}
$$
where $\tau$ is a threshold typically set to $\floor*{\frac{\sum w_i}{2}} + 1$.
\end{enumerate} 

For the sake of simplicity, we refer to the model presented in (ii) as 
\emph{weighted-vote}. One can simplify the model by giving equal weight 
to all $w_i$ (typically $w_i = 1$). We refer to this non-weighted votation 
system as \emph{simple-vote}. 


\guillermo{I thought we needed to add some sort of formulation as overview of what follows. We should revisit the following sections (including the evaluation) and use this terminology to be consistent. I would suggest to change ``majority-vote'' to \emph{simple-vote} and ``ensemble'' to \emph{weighted-vote} in Table \ref{tab:results}... but I'm happy to discuss alternatives.}

% ::::::::::::::::::::::::: % 
\subsection{Feature Engineering}
\label{sec:core:fengineering}
% ::::::::::::::::::::::::: % 

Our work considers a diverse set of features aiming at building a robust 
classification system. The proposed set of features contain elements obtained 
from three different sources: 
(i) structured attributes of the profile referred as \emph{demographics} 
and denoted as $\theta_M$, 
(ii) features extracted from raw images referred as \emph{captions} ($\theta_C$), and 
(iii) features extracted from unstructured text (\emph{description} 
denoted as $\theta_D$). 
Based on the preprocessing described in Section \ref{sec:preliminaries}, 
we extract different type of features as described bellow. 

\begin{itemize}
\item \textbf{Numerical Features} (NF): refers to those attributes from a profile 
that take a quantitative measurement such as the age (18-85) of a person.  
\item \textbf{Categorical Features} (CF): refers to those attributes 
that take a limited number of possible values such as the gender (male or female). 
\item \textbf{Set-based Features} (SBF): refers to those attributes that can take an 
arbitrary number of values and the relationship between sets of attributes is 
relevant (e.g.: words in the description). 
\end{itemize}


We distinguish between two type of categorical features: binary features (BCF), 
and continuous features (CCF). We use both types depending on the setting. 
For instance, the presence or absence of a particular trait, such as the gender, 
is encoded as a binary feature; while numeric properties, such age or occurrences 
of a given trait, are encoded as continuous features. %Continuous features are scaled.
%\guillermo{Check about the age.}

As for the set-based features, we mainly consider sequences of words of arbitrary 
length---namely \emph{ngrams}, where $n$ is the length chosen. Ngrams has been 
widely used in the field of text mining \cite{cavnar1994n} and successfully applied 
to authorship attribution \cite{kevselj2003n}. It is usually desirable to take word sequence of small length (e.g.: two or three) as longer sequences are known to reduce the classification performance \cite{furnkranz1998study}. 

Table \ref{tab:features} shows the set of features proposed categorized by the 
source in the profile. For $\theta_M$ we considered the age, and the 
various location values as numerical values, while the gender, country, ethnicity 
and occupation are categorical. We normalized the occupation to consider about 45 
different occupations including self-employed, military or legal. Note that we 
aggregated some occupations into categories. For instance, the legal category was 
given to occupations ranging from lawyer or attorney to solicitor or judge, to name a 
few. Any other occupation that does not fit into our categories is set as \textit{other}.

\begin{table}[ht]
\centering
\caption{Our proposed set of features.}
\begin{tabular}{llll}
  \hline
 ID & Source & 	Name 		& Type 	\\ 
\hline
\multirow{7}{*}{$\theta_M$} &
\multirow{7}{*}{Demographics}
		  	 		  	& 	Age 		& 	NF 	\\ 
		  	& 		  	&  	Gender 		& 	BCF 	\\ 
		  	& 		  	&  	Latitude 	& 	NF 	\\ 
		  	& 		  	& 	Longitude 	& 	NF 	\\ 
		  	& 		  	& 	Country 	& 	CCF 	\\ 
		  	& 		  	& 	Ethnicity	& 	CCF 	\\ 
		  	& 		  	& 	Occupation 	& 	CCF 	\\ 
\hline
\multirow{3}{*}{$\theta_C$} &
\multirow{3}{*}{Captions}
		  	 		  	& 	\texttt{set}(\emph{entities}) 		& 	BCF 	\\ 
		  	& 		  	& 	\texttt{set}(\emph{actions}) 		& 	BCF 	\\ 
		  	& 		  	& 	\texttt{set}(\emph{modifiers}) 	& 	BCF 	\\ 
\hline
$\theta_S$ 	&
 Descriptions & \texttt{set}(\emph{ngrams}) 	& 	SBF 	\\ 
\hline
\end{tabular}
\label{tab:features}
\end{table}

%Some continuous features are transformed into binary by transforming 
%each possible value into $m$ features, where $m$ is the number of all 
%possible values that the variable can take. 
%\guillermo{I thought it was the case for the demographics but it's not}


As for $\theta_C$, after extracting the most representative caption per 
image, we removed the least informative elements and retained only 
entities (nouns), actions (verbs), and modifiers (adverbs and adjectives). 
Each element in the caption is processed to a common base to reduce 
inflectional forms and derived forms (know as stemming). 
Rather than treating the captions as set-based features, we encode them 
as binary categorical features simply because the order of the actions 
is not relevant in this domain. Captions are rather simple and their structure 
always follows the same pattern. Measuring the presence of a given action and 
the set of objects appearing in the image is itself informative. On the contrary, 
encoding the relationship between the different parts of the speech would 
unnecessarily increase the number of features. 


Finally, we extracted set-based features from the textual content of the 
descriptions ($\theta_S$). We first tokenized the description, removed all 
stop words (words with little lexical content) and stemmed the reminder 
ones. We then extracted ngrams of length \fixme{$n=3$}.
\guillermo{This needs to be confirmed and additional details 
should be added regarding the ngrams.}






% ::::::::::::::::::::::::: % 
\subsection{Prediction Models}
\label{sec:core:model}
% ::::::::::::::::::::::::: % 

We now present three independent classifiers to estimate the presence of 
fraudulent profiles. Each classifier has been designed to effectively model 
a section of the profile (based on $\theta_M$, $\theta_C$ and $\theta_S$ as 
described previously). Available decisions are later combined to provide 
one unanimous output (i.e.: $f = \{\texttt{scam}, \texttt{real}\}$).

The motivation behind the use of three different ensemble classifiers is 
as follows. Profiles in online dating sites are inherently incomplete since 
most of the fields are optional. Some users are jealous about sharing certain 
type of information and some others simply do not find the motivation to 
complete their profile. Thus, any reliable decision system should be able to 
flexibly deal with incomplete profiles. Here, ensemble methods are suitable 
for this. 
%
Another reason behind it is that ensembles often perform better than one 
single classifier \cite{dietterich2000ensemble}. 

%For the purpose of this paper, we focus on sections... We denote  $i \in \set{D, I, S}$... \guillermo{WIP}.

\guillermo{Note that we are finally not combining all features together. If I were to review this paper I'd most likely criticize it... as we might be missing valuable relationships that could happen across sections of the profile (e.g.: demographics and images). Without having empirical results, I have justified our work the best I could. However, feel free to put more flesh on this if considered appropriate.}


%% %% %% %% %%%% %% %% %% %% %% %% %%
\subsubsection*{Demographics Classifier}
%% %% %% %% %%%% %% %% %% %% %% %% %%

$P_M(X = \texttt{scam})$

%% %% %% %% %% %% %% %% %% %% %% %% %%
\subsubsection*{Images Classifier}
%% %% %% %% %% %% %% %% %% %% %% %% %%

$P_I(X = \texttt{scam})$
\guillermo{WIP}

% This framework have been originally proposed to generate captions from images and the output given can be used to train a classifier based on relevant keywords obtained. The main idea is to extract captions from both sets in our dataset (scam and non-scam) and analyse if the context of the images can contribute to the detection of scammers. This could work out nicely If the them found on the images uploaded by the scammers is prevalent (sports, military, doctors, etc). 

%% %% %% %% %% %% %% %% %% %% %% %% %%
\subsubsection*{Descriptions Classifier}
%% %% %% %% %% %% %% %% %% %% %% %% %%

$P_S(X = \texttt{scam})$

%% %% %% %% %% %% %% %% %% %% %% %% %%
\subsubsection*{Ensemble Classifier}
%% %% %% %% %% %% %% %% %% %% %% %% %%


\guillermo{WIP}

The goal of this method is to combine the predictions of the base estimators 
described above to improve the robustness of the classification. Ensemble 
methods are design to construct a decision based on a set of classifiers by 
taking a weighted vote of all available predictions. 



% - Dealing with the absence of a decision (default-to...)
% - Probability Calibration
% - Majority Voting
% - Weights 


$$f(P_M, P_I, P_S) = \{\texttt{scam}, \texttt{real}\}$$


One can find typically two type of ensemble methods: \emph{averaging} and \emph{boosting} methods. 
Our system supports 


averaging their probabilistic prediction, instead of letting each classifier vote for a single class


Boost: The predictions from all of them are then combined through a weighted majority vote (or sum) to produce the final prediction




==> sections/core_CP.tex <==

% -----------------------------------------------
\section{Experimental Set-up}
% -----------------------------------------------
\label{sec:core}

Our approach to identifying profiles that are possibly used by online dating 
scammers to attract and fraud their victims is based on automatic text and image 
categorisation. This involves (1) the compilation of a pre-labelled
dataset (in our case \textsc{scam} versus \textsc{real} profiles),
(2) selecting potentially discriminative features and
(3) building a classification model that can attribute new profiles
automatically to one of the predefined classes with sufficient
reliability. However, building a classification system that is
sufficiently robust to be employed on online dating sites 
is a challenging task for a variety of reasons. 

Firstly, users' online dating behaviour differs greatly from that in other
types of social media (e.g. spontaneous communications, contacting many users with a similar 
or even identical opening line, providing inaccurate profile meta data, migrating conversations to other
media, etc.). As a result, such behaviour -- which is typically considered to be suspicious on other
platforms (cf. \S\ref{sec:related}) -- cannot be used to detect malicious intentions.
Moreover, contrary to other types of online scams, most romance scams do not include any 
scam bots, but are set up by humans who (in many cases) excel at responding to their victim's
idealised romantic beliefs, while hiding their true identity.

In this section, we introduce our approach to automatically identify fraudulent online dating profiles. 
We first describe how we pre-processed the \textsc{Romance Scam} dataset. Because not all profiles contain 
the same information, our work considers a diverse set of features obtained 
from three different sources: 
(i) structured attributes of the profile, 
(ii) features extracted from raw images, and 
(iii) features extracted from unstructured text. 

The results of our experiments are presented in \S\ref{sec:evaluation}.

  
% ::::::::::::::::::::::::: % 
\subsection{Data Pre-processing}
\label{sec:core:dataprep}
% ::::::::::::::::::::::::: % 

As we mentioned above, the data was collected by scraping two sources: \url{scamdiggers.com} 
and \url{datingnmore.com}. The first scraping process resulted in 5,402 scammer profiles. To simulate a 
real-life data distribution on a dating website, we also collected a large random sample of 14,720 real 
dating profiles. 

Next, the dataset was partially cleaned and segmented to support machine learning. More specifically, within the 
original data, many scammers had fields coded with 'or' values where the annotators have combined multiple sightings 
of the same profile using slightly different values for age, occupation, etc. More specifically, the data in the 
\textsc{Romance Scam} dataset has exploded these options into each of the possible combinations. 

Next, each profile was stored 
as an individual single-line JSON file, named according to their page name from the source and was randomly assigned to training, 
test or validation sets, but without allowing any 'duplicated' scam profiles to appear in both sets.

Other cleaning has included standardising the coding of missing data (including adding all variables to all JSON objects) and some 
standardisation of case (but not spelling) on some categorical demographic data. Additionally, all profiles have latitude,longitude 
and country geocoding results added, based on queries using the location field. 

As mentioned above, the data available for scammers and ordinary users differs slightly. Table \ref{table} enumerates the profile variables,
explains their meaning and their availability for each category.

\claudia{Matt: can you copy your table from GitHub here?}


% ::::::::::::::::::::::::: % 
\subsection{Feature Engineering}
\label{sec:core:fengineering}
% ::::::::::::::::::::::::: % 

Based on the pre-processing described in Section \ref{sec:core:dataprep}, 
we extract different type of features as described bellow. 

\begin{itemize}
	\item \textbf{Categorical Features}: refers to those attributes from a profile 
	that take a limited number of possible values such as the gender (male or female) 
	or the age (18-85) of a person. 
	\item \textbf{Set-based Features}: refers to those attributes that can take an 
	arbitrary number of values and the relationship between sets of attributes is 
	relevant (e.g.: words in the description). 
\end{itemize}

We distinguish between two types of categorical features: binary and continuous features. 
We use both types depending on the setting. 
For example, the presence or absence of a particular profile variable (e.g. occupation), 
is encoded as a binary feature. Numeric properties, such as age or occurrences 
of a given variable, are encoded as continuous features. 
\guillermo{Check about the age.}

With regard to the set-based features, we first extracted \emph{Bag-of-Words} features from the profile 
descriptions. Next, 
we extracted all patterns of two and three consecutive words (also called \emph{word
n-grams}, together with \emph{character n-grams}, because these types of features have been successfully 
applied in the field of authorship attribution \cite{kevselj2003n}. We did not perform any stemming, 
standardisation, spelling correction or filtering of any kind, because this lead to a decrease of the 
performance during our preliminary experiments.


Figure~\ref{fig:architecture-general} provides an overview of the pre-processing and feature extraction processes
which prepared the data for the machine learning experiments we describe in Section \S\ref{sec:evaluation}, 
and summarizes the techniques used in each step.

\begin{figure*}[t]
	\includegraphics[width=\textwidth, trim = 20 195 55 35, clip]{architecture-general}
	\caption{Key features extracted from dating profiles.}\label{fig:architecture-general}
\end{figure*}
 


